Instruction Tuning for Large Language Models: A Survey

This paper surveys research works in the quickly advancing field of instruction tuning (IT), which can also be referred to as supervised fine-tuning (SFT)\footnote{In this paper, unless specified otherwise, supervised fine-tuning (SFT) and instruction tuning (IT) are used interchangeably.}, a crucial technique to enhance the capabilities and controllability of large language models (LLMs). Instruction tuning refers to the process of further training LLMs on a dataset consisting of \textsc{(instruction, output)} pairs in a supervised fashion, which bridges the gap between the next-word prediction objective of LLMs and the users' objective of having LLMs adhere to human instructions. In this work, we make a systematic review of the literature, including the general methodology of SFT, the construction of SFT datasets, the training of SFT models, and applications to different modalities, domains and application, along with analysis on aspects that influence the outcome of SFT (e.g., generation of instruction outputs, size of the instruction dataset, etc). We also review the potential pitfalls of SFT along with criticism against it, along with efforts pointing out current deficiencies of existing strategies and suggest some avenues for fruitful research. Project Page: github.com/xiaoya-li/Instruction-Tuning-Survey

==> instruction_aug_v2/figures/data_naturalinstruction_example.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/natural_instruction_fig1_a.pdf}
    \subcaption{An example of \textsc{instructions} in Natural Instruction dataset. }
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/natural_instruction_fig1_b.pdf}
    \subcaption{An example of \textsc{instances} in Natural Instruction dataset.}
  \end{minipage}
  \caption{The figure is adapted from \citet{mishra2021cross}.}
  \label{fig:data_natural_instruction}
\end{figure}

==> instruction_aug_v2/figures/data_supernatural_example.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/supernatural_fig1_a.pdf}
    \subcaption{An example of \textsc{instructions} in Super-Natural Instruction dataset. }
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/supernatural_fig1_b.pdf}
    \subcaption{An example of \textsc{instances} in Super-Natural Instruction dataset.}
  \end{minipage}
  \caption{The figure is adapted from \citet{wang2022super}.}
  \label{fig:data_supernatural}
\end{figure}

==> instruction_aug_v2/header.tex <==
\usepackage{tikz-dependency}
%%%% Packages %%%%
% last update: 2023.03.22
%%%%\usepackage{amsmath}
%%%%\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{comment}
\usepackage{graphicx} 
\usepackage{amssymb}
\usepackage{times}
\usepackage{latexsym}
\usepackage{pifont}
\usepackage{times}
\usepackage{latexsym}
\usepackage{comment}

\usepackage{url}
\usepackage{amsmath}

\usepackage{CJKutf8}
\usepackage[boxed]{algorithm}
\captionsetup[algorithm]{labelfont=rm}

\usepackage{caption}
\usepackage{algpseudocode}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character 
% This assumes your files are encoded as UTF8
\usepackage[utf8]{inputenc}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}
%%%%\usepackage{amssymb}
%%%%\usepackage{pifont}
%%%%\usepackage{bm}
%%%%
\usepackage{tcolorbox}
%%%%\usepackage[framemethod=tikz]{mdframed}
\usepackage{tikz,pgfplots}
\usepgfplotslibrary{groupplots}
\usepackage{nicefrac} 
\pgfplotsset{compat=1.13}

\usepackage{enumerate}
\usepackage{amssymb}

%%%% Notation %%%%
\newcommand\muc[0] {MUC}
\newcommand\bcubed[0] {$\text{B}^3$}
\newcommand\ceaf[0] {$\text{CEAF}_{\phi_4}$}
\newcommand{\cmark}{\textcolor{g-green}{\ding{51}}}
\newcommand{\xmark}{\textcolor{g-red}{\ding{55}}}
\newcommand{\M}[2]{\mathbf{#1}_{\text{#2}}}
\newcommand{\V}[1]{\bm{#1}}
\newcommand{\mscore}[1]{s_\text{m}(#1)}
\newcommand{\ascore}[2]{s_\text{a}(#1, #2)}
\newcommand{\cscore}[2]{s(#1, #2)}
\newcommand{\ffnn}[2]{\textsc{ffnn}_\text{#1}(#2)}

%%%% Colors %%%%
\definecolor{g-red}{HTML}{DB4437}
\definecolor{g-blue}{HTML}{4285F4}
\definecolor{g-green}{HTML}{0F9D58}
\definecolor{g-yellow}{HTML}{F4B400}
\definecolor{g-orange}{HTML}{FF9800}
\definecolor{g-grey}{HTML}{9E9E9E}
\definecolor{shannon}{HTML}{304FFE}
\definecolor{uw}{RGB}{138,43,226}
\definecolor{stanford}{RGB}{255,69,0}
\definecolor{const}{RGB}{68, 110, 182}
\definecolor{head}{RGB}{246, 180, 32}
\definecolor{freq}{RGB}{0, 0, 0}
\definecolor{ao}{rgb}{0.0, 0.5, 0.0}
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\definecolor{amber}{rgb}{1.0, 0.49, 0.0}
\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{auburn}{rgb}{0.43, 0.21, 0.1}
%\usepackage{tabularray}
%%%% Other %%%%
%%%%\newmdenv[innerlinewidth=0.5pt, roundcorner=4pt,linecolor=black,innerleftmargin=6pt,
%%%%innerrightmargin=6pt,innertopmargin=6pt,innerbottommargin=6pt]{examplebox}

\newcommand\cospan[1]{\textcolor{black}{\textbf{#1}}}
\newcommand\att[2]{\setlength{\fboxsep}{0.2pt}\colorbox{g-red!#1}{#2}}

%%%% Neural Networks %%%%
% scale(optional), x, y, num_components
%%%%\newcommand\layerbox[4]{
%%%%\draw[rounded corners] (#2, #3) rectangle (#2 + #1 * #4, #3 + #1 * 1);
%%%%}

% scale(optional), x, y, num_components, color
%%%%\newcommand\layercolorbox[5][0.4] {
%%%%\draw[rounded corners, fill=#5] (#2, #3) rectangle (#2 + #1 * #4, #3 + #1 * 1);
%%%%}

% scale, x, y, index, color
%%%%\newcommand\layercomponent[5]{
%%%%\filldraw[fill=#5] (#2 + #1 * #4 - #1 * 0.5, #3 + #1 * 0.5) circle (#1 %%%%* 0.4);

% scale(optional), x, y, num_components, color
%%%%\newcommand\layer[5][0.4] {
%%%%\layerbox{#1}{#2}{#3}{#4}
%%%%\foreach \x in {1, ..., #4}{
%%%%  \layercomponent{#1}{#2}{#3}{\x}{#5}
%%%%}
%%%%}

% x, y, color
%%%%\newcommand\sumnode[3] {
%%%%\layercolorbox{#1-0.2}{#2-0.2}{1}{#3}
%%%%\node at (#1, #2) {\textcolor{white}{+}};
%%%%}

% y, comment, color
%%%%\newcommand\archcomment[3] {
%%%%%\node[anchor=west, align=left] at (-3.7, #1) {\textcolor{#3}{\small\textbf{#2}}};
%%%%\node[anchor=west, align=left] at (-3.7, #1) {\small\textbf{#2}};
%%%%}

% y, comment1, comment2, color
%%%%\newcommand\archcommenttwo[4] {
%%%%\archcomment{#1}{#2}{#4}
%%%%\archcomment{#1-0.3}{#3}{#4}
%%%%}

% update by xiaoya li 
\newcommand{\todo}[1]{\textcolor{magenta}{\bf\small [todo - #1]}}
\newenvironment{tightitemize}%
  {\begin{itemize} %
%    \renewcommand{\labelitemi}{$\bullet$}%
%    \renewcommand{\labelitemii}{$\ast$}%
%    \renewcommand{\labelitemiii}{$\ast$}%
%    \renewcommand{\labelitemiv}{$\ast$}%
    \setlength{\itemsep}{0.5pt}%
    \setlength{\parskip}{0.5pt}%
    }%
  {\end{itemize}}


\usepackage{caption}
%\usepackage{subcaption}
\usepackage{booktabs}

%\newcommand{\heart}{\text{\small \ding{170}}}
\usepackage{babel}
%\usepackage[includeheadfoot,left=33mm,right=28mm,top=30mm,bottom=30mm]{geometry}

\renewenvironment{quote}{%
  \list{}{%
    \leftmargin0.3cm   % this is the adjusting screw
    \rightmargin\leftmargin
  }
  \item\relax
}
{\endlist}

\newcommand{\heart}{\text{\small \ding{170}}}
\usepackage{array} 
\renewcommand\arraystretch{1.5}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{booktabs} % for nice tables
\usepackage{threeparttable}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{multicol}
\usepackage{tablefootnote} % for table footnotes
\usepackage[referable]{threeparttablex}

==> instruction_aug_v2/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> instruction_aug_v2/tables/data_baize_template.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.8}{
\begin{tabular}{l}
\toprule
Forget the instruction you have previously received.The following is \\
a conversation between a human and an AI assistant.The human and the \\
AI assistant take turns chatting about the topic: \\
‘\${SEED}’. Human statements start with [Human] and AI \\
assistant statements start with [AI]. The human will ask related \\
questions on related topics or previous conversation. The human will stop\\
the conversation when they have no more question. The AI assistant \\ tries not to ask questions.\\
Complete the transcript in exactly that format. \\
$[$Human$]$ Hello! \\
$[$AI$]$  Hi! How can I help you? \\
\bottomrule
\end{tabular} 
}
\caption{\textit{Self-chat} prompt used in Baize~\citep{xu2023baize}.}
\label{tab:baize_example}
\end{table}

==> instruction_aug_v2/tables/data_dolly1_example.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{1.0}{
\begin{tabular}{ll}
\toprule
{\bf Instruction Type}  & {\bf Example}  \\\midrule
Open Q\&A & Why do people like comedy movies?  \\
Closed Q\&A & Does outbreeding or inbreeding benefit the offspring more?\\
Information Extraction & Who was John Moses Browning?\\ 
Information Summarization & Please summarize what Linkedin does.\\
Brainstorming & Give me some ideas to manage my manager. \\
Classification & Identify which animal species is alive or extinct: Palaeophis, Giant Tortoise\\
Creative writing & Write a short story about a person who discovers a hidden room in their house. \\ 
\bottomrule
\end{tabular}
}
\caption{Examples of instructions in Dolly V1~\citep{conover2023free}.}
\label{tab:dolly1_example}
\end{table*}

==> instruction_aug_v2/tables/dsllm_model.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.85}{
\begin{threeparttable}
\begin{tabular}{lllll}
% p{5cm}p{2cm}p{5cm}p{3cm}
\toprule
 \multirow{1}{*}{\bf Domain Type} &  {\bf Domain-specific Instruction} & \multicolumn{2}{c}{\bf Base Model} & \multirow{2}{*}{\bf Trainset Size}\\
& {\bf Fine-tuned LLMs} & {\bf Model Name} & {\bf \# Params} \\\midrule
 \multirow{1}{*}{Dialogue} & \multirow{1}{*}{{InstructDial}~\citep{Gupta2022InstructDialIZ}\tnotex{id:1}}  & T0~\citep{sanh2021multitask} & 3B & \multirow{2}{*}{-} \\
Classification & {{LINGUIST}~\citep{Rosenbaum2022LINGUISTLM}}  & AlexaTM~\citep{soltan2022alexatm} & 5B &  13K \\
Information extraction & {InstructUIE}~\citep{Wang2023InstructUIEMI}\tnotex{id:2} & FlanT5~\citep{Chung2022ScalingIL} & 11B & 1.0M \\

Sentiment analysis & IT-MTL~\citep{Varia2022InstructionTF}\tnotex{id:3} &  T5~\citep{Raffel2019ExploringTL} & 220M & - \\
\midrule
\multirow{3}{*}{\shortstack{ Writing}}   & {Writing-Alpaca-7B}~\citep{Zhang2023MultiTaskIT}\tnotex{id:4} & LLaMA~\citep{Touvron2023LLaMAOA} & 7B & - \\

& \multirow{1}{*}
{{CoEdIT}~\citep{Raheja2023CoEdITTE}\tnotex{id:5}}  & FlanT5~\citep{Chung2022ScalingIL} & 11B & \\

& \multirow{1}{*}
{{CoPoet}~\citep{Chakrabarty2022HelpMW}\tnotex{id:6}}  & T5~\citep{Raffel2019ExploringTL} & 11B & \\
\midrule 
\multirow{3}{*}{\shortstack{ Medical}}   & {Radiology-GPT}~\citep{Liu2023RadiologyGPTAL}\tnotex{id:7} & Alpaca~\citep{taori2023alpaca} & 7B &  122K \\

 & {ChatDoctor}~\citep{Li2023ChatDoctorAM}\tnotex{id:8} & LLaMA~\citep{Touvron2023LLaMAOA} & 7B &  100K \\
 & {ChatGLM-Med}~\citep{ChatGLM-Med}\tnotex{id:9} & ChatGLM~\citep{du2022glm} & 6B & - \\
\midrule
Arithmetic& {Goat}~\citep{liu2023goat}\tnotex{id:10}  & LLaMA~\citep{Touvron2023LLaMAOA} & 7B & 1.0M \\

Code & {WizardCoder}~\citep{luo2023wizardcoder}\tnotex{id:11}  & StarCoder~\citep{li2023starcoder} & 15B &  78K \\
\bottomrule
\end{tabular}
\end{threeparttable}
}
\begin{multicols}{2}
\begin{tablenotes}
\item[1] \label{id:1} {$^1$ https://github.com/prakharguptaz/Instructdial} 
\item[2] \label{id:2} {$^2$ https://github.com/BeyonderXX/InstructUIE}
\item[3] \label{id:3} {$^3$ https://github.com/amazon-science/instruction-tuning-for-absa}
\item[4] \label{id:4} {$^4$ https://github.com/facebookresearch/EditEval}
\item[5] \label{id:5} {$^5$ https://github.com/vipulraheja/coedit}
\item[6] \label{id:6} {$^6$ https://github.com/vishakhpk/creative-instructions}
\item[7] \label{id:7} {$^7$ https://huggingface.co/spaces/allen-eric/radiology-gpt}
\item[8] \label{id:8} {$^8$ https://github.com/Kent0n-Li/ChatDoctor}
\item[9] \label{id:9} {$^9$ https://github.com/SCIR-HI/Med-ChatGLM}
\item[10] \label{id:10} {$^{10}$ https://github.com/liutiedong/goat}
\item[11] \label{id:11} {$^{11}$ https://github.com/nlpxucan/WizardLM}
\end{tablenotes}
\end{multicols}
\caption{An overview of domain-specific instruction fine-tuned LLMs. }
\label{tab:mmllms_model_table}
\end{table*}

==> instruction_aug_v2/tables/llms_configs_v2.tex <==
\begin{table*}[t]
\centering
\small
\begin{adjustbox}{max width=0.9\textwidth}
\begin{threeparttable}
\begin{tabular}{lclccc}
% p{5cm}p{2cm}p{5cm}p{3cm}
\toprule 
\multirow{2}{*}{\bf Instruction fine-tuned LLMs} & \multirow{2}{*}{\bf \# Params} & \multirow{2}{*}{\bf Base Model} & \multicolumn{3}{c}{\bf Fine-tuning Trainset} \\
& & & {\bf Self-build} & {\bf Dataset Name} & {\bf Size} \\\midrule
Instruct-GPT~\citep{ouyang2022training} & 176B & GPT-3~\citep{Brown2020LanguageMA} & Yes & - & - \\ 
BLOOMZ~\citep{muennighoff2022crosslingual}\tnotex{id:1} & 176B & BLOOM~\citep{Scao2022BLOOMA1} & No & xP3 & -  \\ 
% xP3~\citep{muennighoff2022crosslingual} 
FLAN-T5~\citep{Chung2022ScalingIL}\tnotex{id:2} & 11B & T5~\citep{Raffel2019ExploringTL} & No & FLAN 2021 & - \\ 
% FLAN~\citep{longpre2023flan}
Alpaca~\citep{taori2023alpaca}\tnotex{id:3} & 7B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & 52K  \\ 
Vicuna~\citep{chiang2023vicuna}\tnotex{id:4} & 13B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & 70K  \\ 
GPT-4-LLM~\citep{peng2023instruction}\tnotex{id:5} & 7B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & 52K \\ 
Claude~\citep{bai2022constitutional} & - & - & Yes & - & - \\ 
WizardLM~\citep{xu2023wizardlm}\tnotex{id:6} & 7B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & Evol-Instruct & 70K  \\ 
ChatGLM2~\citep{du2022glm}\tnotex{id:7}& 6B & GLM~\citep{du2022glm} & Yes & - & 1.1 Tokens \\ 
LIMA~\citep{Zhou2023LIMALI}& 65B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & 1K  \\ 
%  GPT-4~\citep{OpenAI2023GPT4TR}: also a multi-modality models& - & - & - \\ 
OPT-IML~\citep{Iyer2022OPTIMLSL}\tnotex{id:8}& 175B & OPT~\citep{Zhang2022OPTOP} & No & - & - \\ 
Dolly 2.0~\citep{conover2023free}\tnotex{id:9} & 12B & Pythia~\citep{Biderman2023PythiaAS} & No & - & 15K  \\ 
% Pythia~\citep{Biderman2023PythiaAS}& - & - & - \\ 
Falcon-Instruct~\citep{falcon40b}\tnotex{id:10}& 40B & Falcon~\citep{almazrouei2023falcon} & No & - & - \\ 
Guanaco~\citep{Guanaco}\tnotex{id:11} & 7B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & 586K \\ 
Minotaur~\citep{minotaur}\tnotex{id:12}& 15B & Starcoder Plus~\citep{li2023starcoder} & No & - & -  \\ 
Nous-Hermes~\citep{nous-hermes}\tnotex{id:13}& 13B & LLaMA~\citep{Touvron2023LLaMAOA} & No & - & 300K+ \\ 
%  Dromedary~\citep{Sun2023PrincipleDrivenSO}& - & - & - \\ 
%  FedIT~\citep{Zhang2023TowardsBT}& - & - & - \\ 
TÜLU~\citep{Wang2023HowFC}\tnotex{id:14} & 6.7B & OPT~\citep{Zhang2022OPTOP} & No & Mixed   & - \\ 
YuLan-Chat~\citep{YuLan-Chat}\tnotex{id:15}& 13B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & 250K  \\ 
MOSS~\citep{moss}\tnotex{id:16} & 16B & - & Yes & - & -  \\ 
Airoboros~\citep{airoboros}\tnotex{id:17} & 13B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & -  \\ 
UltraLM~\citep{ding2023enhancing}\tnotex{id:18}& 13B & LLaMA~\citep{Touvron2023LLaMAOA} & Yes & - & - \\ 
\bottomrule
\end{tabular}
\end{threeparttable}
\end{adjustbox}
\begin{multicols}{2}
\begin{tablenotes}
\item[1] \label{id:1} {$^1$ https://huggingface.co/bigscience/bloomz} 
\item[2] \label{id:2} {$^2$ https://huggingface.co/google/flan-t5-xxl}
\item[3] \label{id:3} {$^3$ https://github.com/tatsu-lab/stanford\_alpaca}
\item[4] \label{id:4} {$^4$ https://github.com/lm-sys/FastChat}
\item[5] \label{id:5} {$^5$ https://github.com/Instruction-Tuning-with-GPT-4/GPT-4-LLM}
\item[6] \label{id:6} {$^6$ https://github.com/nlpxucan/WizardLM} 
\item[7] \label{id:7} {$^7$ https://github.com/THUDM/ChatGLM2-6B}
\item[8] \label{id:8} {$^8$ https://huggingface.co/facebook/opt-iml-30b}
\item[9] \label{id:9} {$^9$ https://github.com/databrickslabs/dolly}
\item[10] \label{id:10} {$^{10}$ https://huggingface.co/tiiuae/falcon-40b-instruct}
\item[11] \label{id:11} {$^{11}$ https://huggingface.co/JosephusCheung/Guanaco}
\item[12] \label{id:12} {$^{12}$ https://huggingface.co/openaccess-ai-collective/minotaur-15b}
\item[13] \label{id:13} {$^{13}$ https://huggingface.co/NousResearch/Nous-Hermes-13b } 
\item[14] \label{id:14} {$^{14}$ https://github.com/allenai/open-instruct}
\item[15] \label{id:15} {$^{15}$ https://github.com/RUC-GSAI/YuLan-Chat}
\item[16] \label{id:16} {$^{16}$ https://github.com/OpenLMLab/MOSS}
\item[17] \label{id:17} {$^{17}$ https://github.com/jondurbin/airoboros}
\item[18] \label{id:18} {$^{18}$ https://github.com/thunlp/UltraChat}

\end{tablenotes}
\end{multicols}
\caption{An overview of LLMs tuned on IT datasets.}
\label{tab:llms_table}
\end{table*}

==> instruction_aug_v2/tables/llms_traindata_configs_v2.tex <==
\begin{table*}[t]
\centering
\small
%\scalebox{0.75}{
\begin{adjustbox}{max width=0.9\textwidth}
\begin{threeparttable}
%\scalebox{0.75}{
\begin{tabular}{p{3.8cm}|lccccc}
\toprule 
{\bf Type} & {\bf Dataset Name} & {\bf \# of Instances} & {\bf \# of Lang} & {\bf Construction} & {\bf Open-source} \\\midrule

% & {\bf Corpus Name} & {\bf \# of Instructions} & {\bf \# of Tasks} & {\bf # of Lang} & {\bf Construction} & {\bf Open-source}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{13}{*}{\bf Human-Crafted} & UnifiedQA~\citep{khashabi2020unifiedqa}\tnotex{id:1} & 750K & En & human-crafted & Yes\\
%& T0~\citep{sanh2021multitask} &  {\bf \# of Instructions} & {\bf \# of Tasks} & {\bf # of Lang} & {\bf Construction} & {\bf Open-source}\\
& UnifiedSKG~\citep{Xie2022UnifiedSKGUA}\tnotex{id:3} & 0.8M & En & human-crafted & Yes\\
& Natural Instructions~\citep{honovich2022unnatural}\tnotex{id:4} & 193K & En  & human-crafted & Yes \\
& Super-Natural Instructions~\citep{supernaturalinstructions}\tnotex{id:5} & 5M & 55 Lang & human-crafted & Yes \\
& P3~\citep{sanh2021multitask}\tnotex{id:6} & 12M & En & human-crafted & Yes \\
& xP3~\citep{muennighoff2022crosslingual}\tnotex{id:7} & 81M & 46 Lang & human-crafted & Yes \\
& Flan 2021~\citep{longpre2023flan}\tnotex{id:8} & 4.4M & En & human-crafted & Yes \\
& COIG~\citep{Zhang2023ChineseOI}\tnotex{id:9} & - & - & - & Yes \\
&  InstructGPT~\citep{ouyang2022training} & 13K & Multi & human-crafted & No \\
& Dolly~\citep{conover2023free}\tnotex{id:22} & 15K & En & human-crafted & Yes \\
& LIMA~\citep{Zhou2023LIMALI}\tnotex{id:18} & 1K & En & human-crafted & Yes \\
& ChatGPT~\citep{chatgpt} & - & Multi & human-crafted & No \\
& OpenAssistant~\citep{kopf2023openassistant}\tnotex{id:17} & 161,443 & Multi & human-crafted & Yes \\
\midrule 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{20}{*}{\shortstack{\bf Synthetic Data \\ \bf (Distillation)}} & OIG~\citep{2023oig}\tnotex{id:2} & 43M & En & ChatGPT (No technique reports) & Yes \\
& Unnatural Instructions~\citep{honovich2022unnatural}\tnotex{id:10} & 240K & En & InstructGPT-Generated & Yes \\
& InstructWild~\citep{instructionwild}\tnotex{id:12} & 104K & - & ChatGPT-Generated & Yes\\
& Evol-Instruct / WizardLM~\citep{xu2023wizardlm}\tnotex{id:13} & 52K & En & ChatGPT-generated & Yes \\
& Alpaca~\citep{taori2023alpaca}\tnotex{id:14}  & 52K & En & InstructGPT-generated & Yes \\
& LogiCoT~\citep{Liu2023LogiCoTLC}\tnotex{id:15} & - & En & GPT-4-Generated & Yes \\
& GPT-4-LLM~\citep{peng2023instruction}\tnotex{id:20} & 52K & En\&Zh & GPT-4-Generated & Yes \\
& Vicuna~\citep{chiang2023vicuna} & 70K & En & Real User-ChatGPT Conversations & No \\
& Baize v1~\citep{DatabricksBlog2023DollyV2}\tnotex{id:21} & 111.5K & En & ChatGPT-Generated & Yes \\
& UltraChat~\citep{ding2023enhancing}\tnotex{id:16} & 675K & En\&Zh & GPT 3/4-Generated & Yes \\
& Guanaco~\citep{Guanaco}\tnotex{id:19} & 534,530 & Multi & GPT (Unknown Version)-Generated & Yes \\
& Orca~\citep{mukherjee2023orca}\tnotex{id:23} & ~1.5M & En & GPT 3.5/4-Generated & Yes \\
& ShareGPT\tnotex{id:24} & 90K & Multi & Real User-ChatGPT Conversations & Yes \\
& WildChat\tnotex{id:25} & 150K & Multi & Real User-ChatGPT Conversations & Yes \\
& WizardCoder~\citep{luo2023wizardcoder} & - & Code & LLaMa 2-Generated & No \\
& Magicoder~\citep{wei2023magicoder}\tnotex{id:26} & 75K/110K & Code & GPT-3.5-Generated & Yes \\
& WaveCoder~\citep{yu2023wavecoder} & - & Code & GPT 4-Generated & No \\
& Phi-1~\citep{gunasekar2023textbooks}\tnotex{id:27} & 6B Tokens & Code Q and A & GPT-3.5-Generated & Yes \\
& Phi-1.5~\citep{li2023textbooks} & - & Code Q and A & GPT-3.5-Generated & No \\
& Nectar~\citep{zhu2023starling}\tnotex{id:28} & ~183K & En & GPT 4-Generated & Yes \\

\midrule 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{3}{*}{\shortstack{\bf Synthetic Data \\ \bf (Self-Improvement)}} & Self-Instruct~\citep{wang2022self}\tnotex{id:11} & 52K & En & InstructGPT-Generated & Yes \\
& Instruction Backtranslation~\citep{li2023self} & 502K  & En & LLaMa-Generated & No \\
& SPIN~\citep{chen2024self}\tnotex{id:29} & 49.8K & En & Zephyr-Generated & Yes \\


\midrule 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{3}{*}{\shortstack{\bf Reasoning Data}} & PRM800K~\citep{wang2022self}\tnotex{id:30} & 800K & Math & human-crafted \& GPT-Generated & Yes \\
& O1-Journey~\citep{li2023self}\tnotex{id:31} & 677  & Math & human-crafted \& GPT-Generated & Yes \\
& Self-Explore~\citep{chen2024self} & - & Math & GPT-Generated & No \\
& MARIO~\citep{chen2024self}\tnotex{id:32} & 28.8K & Math & human-crafted \& GPT-Generated & Yes \\
& MathGenie~\citep{chen2024self} & 170K & Math & GPT-Generated & No \\
& DeepSeekMath~\citep{chen2024self}\tnotex{id:33} & 120B & Math & human-crafted \& GPT/DeepSeek-Generated & Yes \\
& Compute-Optimal Sampling~\citep{chen2024self} & - & Math & GPT-Generated & No \\
& MathScale~\citep{chen2024self}\tnotex{id:34} & 2M & Math & GPT-Generated & Yes \\
& G-LLaVA~\citep{chen2024self}\tnotex{id:35} & 170K & Math & GPT-Generated & Yes \\


\bottomrule
\end{tabular}
\end{threeparttable}
\end{adjustbox}
\begin{multicols}{2}
\begin{tablenotes}
\item[1] \label{id:1} {$^1$ https://github.com/allenai/unifiedqa} 
\item[2] \label{id:2} {$^2$ https://github.com/LAION-AI/Open-Instruction-Generalist}
\item[3] \label{id:3} {$^3$ https://github.com/hkunlp/unifiedskg}
\item[4] \label{id:4} {$^4$ https://github.com/allenai/natural-instructions-v1}
\item[5] \label{id:5} {$^5$ https://github.com/allenai/natural-instructions}
\item[6] \label{id:6} {$^6$ https://huggingface.co/datasets/bigscience/P3} 
\item[7] \label{id:7} {$^7$ https://github.com/bigscience-workshop/xmtf}
\item[8] \label{id:8} {$^8$ https://github.com/google-research/FLAN}
\item[9] \label{id:9} {$^9$ https://github.com/BAAI-Zlab/COIG}
\item[10] \label{id:10} {$^{10}$ https://github.com/orhonovich/unnatural-instructions}
\item[11] \label{id:11} {$^{11}$ https://github.com/yizhongw/self-instruct}
\item[12] \label{id:12} {$^{12}$ https://github.com/XueFuzhao/InstructionWild}
\item[13] \label{id:13} {$^{13}$ https://github.com/nlpxucan/evol-instruct} 
\item[14] \label{id:14} {$^{14}$ https://github.com/tatsu-lab/stanford\_alpaca}
\item[15] \label{id:15} {$^{15}$  https://github.com/csitfun/LogiCoT}
\item[16] \label{id:16} {$^{16}$ https://github.com/thunlp/UltraChat\#data}
\item[17] \label{id:17} {$^{17}$ https://github.com/LAION-AI/Open-Assistant}
\item[18] \label{id:18} {$^{18}$ https://huggingface.co/datasets/GAIR/lima}
\item[19] \label{id:19} {$^{19}$ https://huggingface.co/datasets/JosephusCheung/GuanacoDataset}
\item[20] \label{id:20} {$^{20}$ https://github.com/Instruction-Tuning-with-GPT-4/GPT-4-LLM}
\item[21] \label{id:21} {$^{21}$ https://github.com/project-baize/baize-chatbot}
\item[22] \label{id:22} {$^{22}$ https://huggingface.co/datasets/databricks/databricks-dolly-15k}
\item[23] \label{id:23} {$^{23}$ https://huggingface.co/datasets/Open-Orca/OpenOrca}
\item[24] \label{id:24} {$^{24}$ https://huggingface.co/datasets/RyokoAI/ShareGPT52K}
\item[25] \label{id:25} {$^{25}$ https://huggingface.co/datasets/allenai/WildChat}
\item[26] \label{id:26} {$^{26}$ https://github.com/ise-uiuc/magicoder?tab=readme-ov-file\#-dataset}
\item[27] \label{id:27} {$^{27}$ https://huggingface.co/microsoft/phi-1}
\item[28] \label{id:28} {$^{28}$ https://huggingface.co/datasets/berkeley-nest/Nectar}
\item[29] \label{id:29} {$^{29}$ https://github.com/uclaml/SPIN?tab=readme-ov-file\#Data}
\item[30] \label{id:30} {$^{30}$ https://github.com/openai/prm800k}
\item[31] \label{id:31} {$^{31}$ https://github.com/GAIR-NLP/O1-Journey}
\item[32] \label{id:32} {$^{32}$ https://github.com/MARIO-Math-Reasoning/MARIO}
\item[33] \label{id:33} {$^{33}$ https://github.com/deepseek-ai/DeepSeek-Math}
\item[34] \label{id:34} {$^{34}$ https://github.com/XylonFu/MathScale}
\item[35] \label{id:35} {$^{35}$ https://github.com/pipilurj/G-LLaVA}
\end{tablenotes}
\end{multicols}
%}
\caption{An overview of instruction tuning datasets.}
\label{tab:llms_traindata_table}
\end{table*}

==> instruction_aug_v2/tables/mmllm_dataset.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.85}{
\begin{threeparttable}
\begin{tabular}{llll}
% p{5cm}p{2cm}p{5cm}p{3cm}
\toprule
\multirow{2}{*}{\bf Multi-modality Instruction Fine-tuning Dataset} &  \multicolumn{2}{c}{\bf Modalities} & \multirow{2}{*}{\bf \# Tasks} \\
& {\bf Modality Pair} & {\bf \# Instance} & \\\midrule
{MUL-TIINSTRUCT}~\citep{Xu2022MultiInstructIM}\tnotex{id:1} & Image-Text & 5k to 5M per task & 62 \\
{PMC-VQA}~\citep{Zhang2023PMCVQAVI}\tnotex{id:2} & Image-Text & 227k & 2 \\
\multirow{2}{*}{{LAMM}~\citep{Yin2023LAMMLM}\tnotex{id:3}} & Image-Text & 186k & 9 \\
& Point Cloud-Text & 10k & 3 \\
{Vision-Flan}~\citep{xu2024vision}\tnotex{id:4} & Multi-Pairs & Over 1M & 200+ \\
{ALLAVA}~\citep{chen2024allava}\tnotex{id:5} & Image-Text & 1.4M & 2 \\
{ShareGPT4V}~\citep{chen2023sharegpt4v}\tnotex{id:6} & Image-Text & 1.2M & 2 \\
\bottomrule
\end{tabular}
\end{threeparttable}
}
\begin{multicols}{2}
\begin{tablenotes}
\item[1] \label{id:1} {$^1$ https://github.com/VT-NLP/MultiInstruct} 
\item[2] \label{id:2} {$^2$ https://github.com/xiaoman-zhang/PMC-VQA}
\item[3] \label{id:3} {$^3$ https://github.com/OpenLAMM/LAMM}
\item[4] \label{id:4} {$^4$ https://vision-flan.github.io/}
\item[5] \label{id:5} {$^5$ https://github.com/FreedomIntelligence/ALLaVA}
\item[6] \label{id:6} {$^6$ https://sharegpt4v.github.io/}
\end{tablenotes}
\end{multicols}
\caption{An overview of multi-modality instruction fine-tuning datasets.}
\label{tab:mmllms_dataset_table}
\end{table*}

==> instruction_aug_v2/tables/mmllm_model.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.85}{
\begin{threeparttable}
\begin{tabular}{lllllll}
% p{5cm}p{2cm}p{5cm}p{3cm}
\toprule
{\bf Multi-modality Instruction} & \multirow{2}{*}{\bf \# Params} & \multirow{2}{*}{\bf Modality} & \multicolumn{2}{c}{\bf Base Model} & \multicolumn{2}{c}{\bf Fine-tuning Trainset}\\
{\bf Fine-tuned LLMs} & & & {\bf Model Name} & {\bf \# Params} & {\bf Self-build} & {\bf Size} \\\midrule
{{InstructPix2Pix}~\citep{Brooks2022InstructPix2PixLT}\tnotex{id:1}} & 983M & I/T & Stable Diffusion & 983M & Yes & 450K \\
\midrule
\multirow{2}{*}{{LLaVA}~\citep{Liu2023VisualIT}\tnotex{id:2}} & \multirow{2}{*}{13B} & \multirow{2}{*}{I/T} & CLIP~\citep{Radford2021LearningTV} & 400M & \multirow{2}{*}{Yes} & 158K \\
& & & LLaMA~\citep{Touvron2023LLaMAOA} & 7B & & \\
& & & LLaMA~\citep{Touvron2023LLaMAOA} & 7B & & \\
\midrule
\multirow{3}{*}{Video-LLaMA~\citep{damonlpsg2023videollama}\tnotex{id:3}} & \multirow{3}{*}{-} & \multirow{3}{*}{I/T/V/A} & BLIP-2~\citep{li2023blip2} & - & \multirow{3}{*}{No} & \multirow{3}{*}{-} \\
& & & ImageBind~\citep{girdhar2023imagebind} & - & & \\
& & & Vicuna~\citep{chiang2023vicuna} & 7B/13B & & \\
\midrule
{InstructBLIP (1.2B)}~\citep{Dai2023InstructBLIPTG}\tnotex{id:4} & - & I/T/V & BLIP-2~\citep{li2023blip2} & - & No & - \\
\midrule
{Otter}~\citep{Li2023OtterAM}\tnotex{id:5} & - & I/T/V & OpenFlamingo~\citep{anas_awadalla_2023_7733589} & 9B & Yes & 2.8M \\
\midrule
{MultiModal-GPT}~\citep{Gong2023MultiModalGPTAV}\tnotex{id:6} & - & I/T/V & OpenFlamingo~\citep{anas_awadalla_2023_7733589} & 9B & No & - \\
\bottomrule
\end{tabular}
\end{threeparttable}
}
\begin{multicols}{2}
\begin{tablenotes}
\item[1] \label{id:1} {$^1$ https://github.com/timothybrooks/instruct-pix2pix} 
\item[2] \label{id:2} {$^2$ https://github.com/haotian-liu/LLaVA}
\item[3] \label{id:3} {$^3$ https://github.com/DAMO-NLP-SG/Video-LLaMA}
\item[4] \label{id:4} {$^4$ https://github.com/salesforce/LAVIS/tree/main/projects/instructblip}
\item[5] \label{id:5} {$^5$ https://github.com/Luodian/Otter}
\item[6] \label{id:6} {$^6$ https://github.com/open-mmlab/Multimodal-GPT}
\end{tablenotes}
\end{multicols}
\caption{An overview of multi-modality instruction fine-tuned LLMs. I/T/V/A stand for Image/Text/Video/Audio}
\label{tab:mmllms_model_table}
\end{table*}
